CHIMERA: Adaptive Cache Injection and Semantic Anchor Prompting for Zero-shot Image Morphing with Morphing-oriented Metrics

Recent diffusion-based image morphing methods typically interpolate inverted latents and reuse limited conditioning signals, which often yields unstable intermediates for heterogeneous endpoint pairs. In particular, (i) feature reuse is usually partial or non-adaptive, leading to abrupt structural changes or over-smoothing, and (ii) text conditions are commonly obtained independently per endpoint and then interpolated, which can introduce incompatible semantics. We present CHIMERA, a novel zero-shot diffusion morphing framework that addresses both issues via inversion-guided denoising with complementary feature reuse and text conditioning. Adaptive Cache Injection (ACI) caches a broader set of multi-scale diffusion features beyond Key-Value-only reuse during DDIM inversion, and re-injects them with layer- and timestep-aware scheduling to stabilize denoising and enable gradual fusion. Semantic Anchor Prompting (SAP) uses a VLM to generate a shared anchor-prompt and anchor-conditioned endpoint prompts, and injects the anchor into cross-attention to improve intermediate semantic coherence. Finally, we propose Global-Local Consistency Score (GLCS), a morphing-oriented metric that jointly captures global domain harmonization and local transition smoothness. Extensive experiments and a user study show that CHIMERA produces smoother and more semantically consistent morphing results than prior methods, while remaining efficient and applicable across diverse diffusion backbones without retraining.

==> sec/X_suppl_freq_analysis.tex <==

% \begin{figure}
%     \centering
%     \includegraphics[width=1.0\textwidth]{./figs/another_backbone_freq_analysis.pdf}
%     \caption{\textbf{Frequency analysis on another backbone.} (i) and (iii) show the layer-wise frequency characteristics of a given diffusion model, while (ii) and (iv) present the timestep-wise frequency characteristics. In each plot, the orange line represents high-frequency components and the blue line represents low-frequency components.}
%     \label{fig:another_backbone_freq} 
% \end{figure}


% \section{Further Analysis on Another Backbone}\label{sp_sec:freq_analysis}

% In this section, we provide additional analyses for the experiments presented in \cref{exp:further_analysis}. 
% In \cref{Sec:PreNObs}, we analyzed diffusion features from a frequency perspective and presented observations that motivate adaptive feature injection based on layer-wise and timestep-wise characteristics. 
% Here, we extend the same frequency-based analysis to other diffusion models to demonstrate that CHIMERA with ACI can generalize to different architectures.

% The analysis in \cref{fig:freq_analysis} focuses on layer- and timestep-wise characteristics of SD~2.1~\cite{rombach2022high}. 
% In this section, we extend the analysis to other U-Net-based diffusion models, including SD~1.4, SD~1.5, and SD~2, as well as larger models such as SDXL~\cite{podell2023sdxl} and the DiT-based model FLUX~\cite{peebles2023scalable,labs2025flux}. 
% As shown in \cref{fig:another_backbone_freq}~(a)-(c), U-Net-based diffusion models share very similar layer structures and therefore exhibit layer- and timestep-wise characteristics that are largely consistent with those observed in SD~2.1 (\cref{fig:another_backbone_freq}~(d)). 
% Based on this observation, applying CHIMERA leads to consistent performance improvements across these models, as reported in \cref{tab:backbone_comparison}.

% As shown in \cref{fig:another_backbone_freq}~(e), SDXL exhibits frequency characteristics similar to those of SD~2.1, although the number of layers differs from that of SD~2.1. 
% To further demonstrate that CHIMERA is not limited to U-Net-based architectures, we extend the analysis to the diffusion transformer model FLUX (\cref{fig:another_backbone_freq}~(f)). 
% As noted in prior DiT-based studies~\cite{chang2025sparsedit, yu2024representation}, early layers of DiT mainly capture low-frequency components, while later layers focus on high-frequency details; similarly, early timesteps tend to generate low-frequency structures, while later timesteps refine high-frequency details. 
% These properties are also reflected in \cref{fig:another_backbone_freq}~(f). Based on these observations, applying CHIMERA to both SDXL and FLUX results in consistent performance improvements, as shown in \cref{tab:backbone_comparison}. 
% These results demonstrate that CHIMERA is not limited to a specific backbone and can be effectively extended to a wide range of diffusion-based models.


==> tables/another_backbone.tex <==
\begin{table}[t!]
\centering

% ---------------- LEFT (Backbone table) ----------------
\begin{minipage}[t]{0.48\textwidth}
\centering
\caption{\textbf{Performance comparison across different diffusion backbones.} 
Evaluation on the target benchmark using FID-local, FID-global, LPIPS, PPL, and GLCS.}
\label{tab:backbone_comparison}

\vspace{0.15cm}

\small
\setlength{\tabcolsep}{5pt}
\resizebox{\linewidth}{!}{%
\begin{tabular}{l c c c c c}
\toprule
\textbf{Exp name} 
& $\mathrm{FID}_{\text{local}}\downarrow$ 
& $\mathrm{FID}_{\text{global}}\downarrow$ 
& LPIPS$\downarrow$ 
& PPL$\downarrow$ 
& GLCS$\uparrow$ \\
\midrule
SD1.4 & 180.237 & 91.003 & 1.782 & 0.300 & 86.924 \\
SD1.4 + CHIMERA & 176.673 & 90.593 & 1.699 & 0.283 & 87.311 \\
SD1.5 & 174.803 & 89.842 & 1.724 & 0.297 & 86.929 \\
SD1.5 + CHIMERA & 172.954 & 88.914 & 1.697 & 0.283 & 87.037 \\
SD2 & 187.790 & 97.053 & 1.667 & 0.280 & 87.741 \\
SD2 + CHIMERA & 185.239 & 95.104 & 1.659 & 0.277 & 88.001 \\
\midrule
SDXL & 209.974 & 101.715 & 2.218 & 0.370 & 84.809 \\
SDXL + CHIMERA & 203.880 & 100.345 & 2.156 & 0.359 & 84.959 \\
\midrule
FLUX & 167.256 & 85.326 & 1.566 & 0.273 & 88.253 \\
FLUX + CHIMERA & 157.780 & 80.826 & 1.552 & 0.259 & 89.983 \\
\bottomrule
\end{tabular}
}
\end{minipage}
\hfill
% ---------------- RIGHT (two stacked tables) ----------------
\begin{minipage}[t]{0.48\textwidth}
\centering

% ---- SAP ablation ----
\caption{\textbf{Ablation on anchor-correlated prompt triplet for SAP.}
Independent endpoint prompts, anchor-conditioned endpoint prompts, and the full anchor-correlated prompt triplet are compared.}
\label{tab:sap_prompt_ablation}

\vspace{0.05cm} % 간격 대폭 축소

% 오른쪽 표의 행간 압축
\renewcommand{\arraystretch}{0.85} 
\scriptsize
\resizebox{\linewidth}{!}{%
\begin{tabular}{l c c c c c}
\toprule
Method & FID$_{\text{local}}\downarrow$ & FID$_{\text{global}}\downarrow$ & LPIPS$\downarrow$ & PPL$\downarrow$ & GLCS$\uparrow$ \\
\midrule
(a) Base$+$per-image prompts & 330.077 & 191.914 & 1.997 & 0.333 & 85.422 \\
(b) Base$+$paired prompts & 255.000 & 144.973 & 2.025 & 0.338 & 87.198 \\
(c) Base$+$SAP & \textcolor{blue}{\underline{209.862}} & \textcolor{blue}{\underline{102.401}} & \textcolor{blue}{\underline{1.907}} & \textcolor{blue}{\underline{0.318}} & \textcolor{blue}{\underline{88.0756}} \\
(d) \textbf{CHIMERA (Ours)} & \textcolor{red}{\textbf{161.054}} & \textcolor{red}{\textbf{82.308}} & \textcolor{red}{\textbf{1.576}} & \textcolor{red}{\textbf{0.263}} & \textcolor{red}{\textbf{88.079}} \\
\bottomrule
\end{tabular}
}

\vspace{0.15cm} % 두 테이블 사이 간격 대폭 축소 (기존 0.35cm)

% ---- runtime table ----
\caption{\textbf{Computational cost comparison.} Runtime, TFLOPs, and learnable parameters.}
\label{tab:runtime_flops}

\vspace{0.05cm} % 간격 대폭 축소

\renewcommand{\arraystretch}{0.85} % 행간 압축 동일 적용
\scriptsize
\resizebox{\linewidth}{!}{%
\begin{tabular}{l c c c}
\toprule
Model & Runtime (s)$\downarrow$ & TFLOPs (T)$\downarrow$ & Learnable (M)$\downarrow$ \\
\midrule
IMPUS & 478.91 & 678.03 & 0.598 \\
DiffMorpher & 96.32 & 554.07 & 6.640 \\
FreeMorph & \textcolor{blue}{\underline{30.66}} & \textcolor{blue}{\underline{426.38}} & \textcolor{red}{\textbf{0}} \\
\textbf{CHIMERA (Ours)} & \textcolor{red}{\textbf{12.36}} & \textcolor{red}{\textbf{213.02}} & \textcolor{red}{\textbf{0}} \\
\bottomrule
\end{tabular}
}

\end{minipage}

\end{table}

==> tables/efficiency.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{6pt}
\begin{tabular}{l c c c}
\toprule
\textbf{Model} 
& \textbf{Runtime (s)$\downarrow$} 
& \textbf{TFLOPs (T)$\downarrow$} 
& \textbf{Learnable (M)$\downarrow$} \\
\midrule

IMPUS 
& 478.91 
& 678.03 
& 0.598 \\

DiffMorpher 
& 96.32 
& 554.07 
& 6.640 \\

FreeMorph 
& \textcolor{blue}{\underline{30.66}}
& \textcolor{blue}{\underline{426.38}} 
&\textcolor{red}{\textbf{0}} \\

\textbf{CHIMERA (Ours)} 
& \textcolor{red}{\textbf{12.36} }
& \textcolor{red}{\textbf{213.02}}
& \textcolor{red}{\textbf{0}} \\

\bottomrule
\end{tabular}
\caption{\textbf{Computational cost comparison.} Runtime, TFLOPs, and learnable parameters (Learnable).}
\label{tab:runtime_flops}
\end{table}

==> tables/ltm.tex <==
\begin{table}[t]
\centering
\caption{Ablation study on Layer- and Timestep-wise Frequency Matching (LTM).}
\small
\setlength{\tabcolsep}{6pt}
\begin{tabular}{l c c c c c}
\toprule
LTM 
& $\mathrm{FID}_{\text{local}}\downarrow$ 
& $\mathrm{FID}_{\text{global}}\downarrow$ 
& LPIPS$\downarrow$ 
& PPL$\downarrow$ 
& GLCS$\uparrow$ \\
\midrule
$\times$
& 182.2786 
& 92.8293 
& 1.6168 
& 0.2695 
& 0.874923 \\
$\checkmark$
& \textcolor{red}{\textbf{161.0539}} 
& \textcolor{red}{\textbf{82.3081}} 
& \textcolor{red}{\textbf{1.5756}} 
& \textcolor{red}{\textbf{0.2626}} 
& \textcolor{red}{\textbf{88.0791}} \\
\bottomrule
\end{tabular}
\label{tab:ltm_ablation}
\end{table}

==> tables/supple_idm.tex <==
% \begin{table}[t]
% \centering
% \begin{minipage}{0.48\columnwidth}
% \caption{\textbf{Quantitative evaluation with respect to the IDM.} We fix the inversion timesteps while performing injections at multiple denoising timesteps.}
% \centering
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{l c c c c c}
% \toprule
% \multicolumn{6}{c}{IDM Ablation - Fixed Inversion Timestep} \\
% \midrule
%  & $\mathrm{FID}_{\text{local}}\downarrow$ 
%  & $\mathrm{FID}_{\text{global}}\downarrow$ 
%  & LPIPS$\downarrow$ 
%  & PPL$\downarrow$ 
%  & GLCS$\uparrow$ \\
% \midrule
% (a) \textbf{Ours}
%     & \textcolor{red}{\textbf{161.054}} 
%     & \textcolor{red}{\textbf{82.308}} 
%     & \textcolor{red}{\textbf{1.576}}
%     & \textcolor{red}{\textbf{0.263}}
%     & \textcolor{red}{\textbf{88.079}} \\
% (b) Early
%     & \textcolor{blue}{\underline{186.030}} 
%     & \textcolor{blue}{\underline{93.002}} 
%     & 1.813 
%     & 0.300 
%     & 87.784 \\
% (c) Mid
%     & 196.437 
%     & 97.327 
%     & 1.764
%     & 0.303
%     & \textcolor{blue}{\underline{87.929}} \\
% (d) Late
%     & 205.031
%     & 101.490
%     & \textcolor{blue}{\underline{1.726}} 
%     & \textcolor{blue}{\underline{0.295}} 
%     & 87.124 \\
% \bottomrule
% \end{tabular}
% }
% \label{table:sp_idm_1}
% \end{minipage}
% \hfill
% \begin{minipage}{0.48\columnwidth}
% \caption{\textbf{Quantitative evaluation with respect to the IDM.} We fix the denoising timesteps while extracting multiple inversion timesteps.}
% \centering
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{l c c c c c}
% \toprule
% \multicolumn{6}{c}{IDM Ablation - Fixed Denoising Timestep} \\
% \midrule
%  & $\mathrm{FID}_{\text{local}}\downarrow$ 
%  & $\mathrm{FID}_{\text{global}}\downarrow$ 
%  & LPIPS$\downarrow$ 
%  & PPL$\downarrow$ 
%  & GLCS$\uparrow$ \\
% \midrule
% (a) \textbf{Ours}
%     & \textcolor{red}{\textbf{161.054}} 
%     & \textcolor{red}{\textbf{82.308}} 
%     & \textcolor{red}{\textbf{1.576}} 
%     & \textcolor{red}{\textbf{0.263}} 
%     & \textcolor{red}{\textbf{88.079}} \\
% (b) Early
%     & \textcolor{blue}{\underline{195.827}} 
%     & \textcolor{blue}{\underline{99.192}} 
%     & 1.858 
%     & 0.310 
%     & \textcolor{blue}{\underline{86.036}} \\
% (c) Mid
%     & 204.923 
%     & 102.100 
%     & 1.691
%     & 0.271 
%     & 85.306 \\
% (d) Late
%     & 206.036 
%     & 102.629 
%     & \textcolor{blue}{\underline{1.690}} 
%     & \textcolor{blue}{\underline{0.269}} 
%     & 85.176 \\
% \bottomrule
% \end{tabular}
% }
% \label{table:sp_idm_2}
% \end{minipage}
% \end{table}

\begin{table}[t]
\centering
\caption{Quantitative evaluation with respect to the IDM. We fix the inversion timesteps while performing injections at multiple denoising timesteps.}
\label{table:sp_idm_1}

\resizebox{0.9\columnwidth}{!}{%
\begin{tabular}{l c c c c c}
\toprule
\multicolumn{6}{c}{IDM Ablation - Fixed Inversion Timestep} \\
\midrule
 & $\mathrm{FID}_{\text{local}}\downarrow$ 
 & $\mathrm{FID}_{\text{global}}\downarrow$ 
 & LPIPS$\downarrow$ 
 & PPL$\downarrow$ 
 & GLCS$\uparrow$ \\
\midrule
(a) \textbf{Ours}
    & \textcolor{red}{\textbf{161.054}} 
    & \textcolor{red}{\textbf{82.308}} 
    & \textcolor{red}{\textbf{1.576}}
    & \textcolor{red}{\textbf{0.263}}
    & \textcolor{red}{\textbf{88.079}} \\
(b) Early
    & \textcolor{blue}{\underline{186.030}} 
    & \textcolor{blue}{\underline{93.002}} 
    & 1.813 
    & 0.300 
    & 87.784 \\
(c) Mid
    & 196.437 
    & 97.327 
    & 1.764
    & 0.303
    & \textcolor{blue}{\underline{87.929}} \\
(d) Late
    & 205.031
    & 101.490
    & \textcolor{blue}{\underline{1.726}} 
    & \textcolor{blue}{\underline{0.295}} 
    & 87.124 \\
\bottomrule
\end{tabular}%
}
\end{table}


\begin{table}[t]
\centering
\caption{Quantitative evaluation with respect to the IDM.
We fix the denoising timesteps while extracting multiple inversion timesteps.}
\label{table:sp_idm_2}

\resizebox{0.9\columnwidth}{!}{%
\begin{tabular}{l c c c c c}
\toprule
\multicolumn{6}{c}{IDM Ablation - Fixed Denoising Timestep} \\
\midrule
 & $\mathrm{FID}_{\text{local}}\downarrow$ 
 & $\mathrm{FID}_{\text{global}}\downarrow$ 
 & LPIPS$\downarrow$ 
 & PPL$\downarrow$ 
 & GLCS$\uparrow$ \\
\midrule
(a) \textbf{Ours}
    & \textcolor{red}{\textbf{161.054}} 
    & \textcolor{red}{\textbf{82.308}} 
    & \textcolor{red}{\textbf{1.576}} 
    & \textcolor{red}{\textbf{0.263}} 
    & \textcolor{red}{\textbf{88.079}} \\
(b) Early
    & \textcolor{blue}{\underline{195.827}} 
    & \textcolor{blue}{\underline{99.192}} 
    & 1.858 
    & 0.310 
    & \textcolor{blue}{\underline{86.036}} \\
(c) Mid
    & 204.923 
    & 102.100 
    & 1.691
    & 0.271 
    & 85.306 \\
(d) Late
    & 206.036 
    & 102.629 
    & \textcolor{blue}{\underline{1.690}} 
    & \textcolor{blue}{\underline{0.269}} 
    & 85.176 \\
\bottomrule
\end{tabular}%
}
\end{table}

==> tables/user_study.tex <==
\begin{wraptable}{r}{0.3\columnwidth}
    \vspace{-1em} % 상단 텍스트와의 여백 미세 조정
    \centering
    % \linewidth를 넣어 wraptable에 할당된 너비(0.45\columnwidth)에 표를 딱 맞춤
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{l c}
        \toprule
        \textbf{Model} & \textbf{Overall Quality}$\uparrow$ \\
        \midrule
        IMPUS & 3.11 $\pm$ 2.11 \\
        DiffMorpher & \textcolor{blue}{$\underline{3.43\pm1.34}$} \\
        FreeMorph & $2.92 \pm 1.21$ \\
        CHIMERA & \textcolor{red}{\textbf{3.61}} \textcolor{red}{$\mathbf{\pm}$} \textcolor{red}{\textbf{1.14}} \\
        \bottomrule
    \end{tabular}%
    }
    \caption{\textbf{User study results.} Overall quality scores (mean $\pm$ std).}
    \label{tab:main_quan_user_study}
    \vspace{-0.5cm} % 하단 여백 조정
\end{wraptable}
